Hybrid Tendon and Ball Chain Continuum Robots for Enhanced Dexterity in Medical Interventions

A hybrid continuum robot design is introduced that combines a proximal tendon-actuated section with a distal telescoping section comprised of permanent-magnet spheres actuated using an external magnet. While, individually, each section can approach a point in its workspace from one or at most several orientations, the two-section combination possesses a dexterous workspace. The paper describes kinematic modeling of the hybrid design and provides a description of the dexterous workspace. We present experimental validation which shows that a simplified kinematic model produces tip position mean and maximum errors of 3% and 7% of total robot length, respectively.

==> sections/abstract.tex <==
A hybrid continuum robot design is introduced that combines a proximal tendon-actuated section with a distal telescoping section comprised of permanent-magnet spheres actuated using an external magnet. While, individually, each section can approach a point in its workspace from one or at most several orientations, the two-section combination possesses a dexterous workspace. The paper describes kinematic modeling of the hybrid design and provides a description of the dexterous workspace. We present experimental validation which shows that the presented model's maximum and mean errors are 12.1\% and 13.4\% of total robot length, respectively, in predicting the robot's tip position.


==> sections/experimental_analysis.tex <==
\begin{figure}[t]
    \centering
    \includegraphics{figures/exp_setup.png}
    \caption{Description of the experimental setup.}
    \label{fig:exp_setup}
\end{figure}

We conducted experiments to validate the kinematic model of Section II and to demonstrate the dexterous workspace derived in Section IV.  The data was collected using the setup in Fig. \ref{fig:exp_setup}, consisting of two orthogonal cameras (webcam C920, Logitech, US) placed in the direction of the points of view (POV) indicated in figure, i.e. from the front and top of the setup.

The tendon-actuated tube was 10.16cm (4 inch) long with the tendon positioned upwards (in the $\pmb x$ direction). 
The tube is composed of two layers: an inner layer of PTFE (polytetrafluoroethylene), an outer layer made of PEBAX (a modified polyamide). A braid made of Stainless Steel 304, is placed between them. The tendon runs the entire length between the outer layer and the braid. 

The ball chain was composed of ten N42 magnetic spheres of diameter 3.175mm (1/8inch), mass 0.13g and remanence 1.32T. This was the smallest strong spherical permanent magnet commercially available (K\&J Magnetics, USA).
An external N52 cylindrical magnet (76.2mm diameter, 38.1mm long, 1.48T remanence) was mounted on a rotatory stage so that it could be precisely positioned with respect to the robot, and its dipole direction could be precisely controlled.

The tube was loaded with no load (0Kg), medium load (0.4Kg) and max load (1.4Kg), by hanging weights over pulleys at the proximal end of the tendon. The maximum load was selected to achieve a bending angle of 90$^\circ$ at the tube's tip. We repeated the experiments with the same loads while extending ball chains of four and eight balls, and rotating the external magnet to four orientations: $\pm \pmb y, \ \pm \pmb z$. The overall set of data used for validation included 24 different configurations. We also collected data (three repetitions) with the tube without internal magnetic balls and used it to compute the elastic modulus of the tube, found to be approximately 4.10GPa, and a shear modulus of 34.13MPa. The tube was observed to retain a curvature of 56.4mm (radius of curvature) when the tendon load was removed. Also, the plane of bending differed from the anticipated vertical plane by an angle of $-26.8^\circ$ rotation around the $\pmb z$ axis from the $\pmb x$ direction. 

The tubes' center line was extracted from the images using the \emph{active contour} and \emph{skeletonizing} operations from the Matlab Image Processing Toolbox. The position of each ball was found \emph{imfindcircles}. The data was converted from the image space to the world space by calibrating each camera using the Matlab \emph{camera calibrator} app; the calibration error was found to be of 1.20px for the front camera and 1.46px for the top camera.


\subsection{Kinematic Model Evaluation}
\begin{figure}
    \centering
    \includegraphics[width = 0.75\columnwidth]{figures/res_pics.png}
    \caption{Front view of experimental results for: (a) smallest error; (b) highest error.}
    \label{fig:res_pics}
\end{figure}

We evaluated the kinematic model of Section II by comparing the experimental data with model predictions. To assess the assumption that the ball chain does not affect tube shape, we computed the error for both tube tip position and ball chain tip position. 

While the tube's centerline was accurately extracted from the images as described above, the tip of the tube was not accurately identified from the images. In contrast, the centers of all extended balls were accurately determined. Therefore, we used the center position of the proximal extended ball as a proxy for tube tip position in order to compute tube modeling error. The center position of the distal ball was used to assess overall error in the combined tube and ball chain model. 

To validate the assumption of decoupling between magnetic ball chain and tube, we computed the error between the tip of the tube during the experiments and its average position during loading experiments without magnetic balls. For each loading condition, we compute the average position of the tube's tip and compare to the one measured without magnetic interaction (no balls and applied field, average over three repetitions). We found an average error of 6.2mm (max 8.5mm), which is comparable to the size of the tip of the catheter (6mm), thus within the error of the segmentation algorithm. Therefore, we can notice negligible interaction between the tendon-actuated and magnetically-actuated sections of the robot. 

Table \ref{table} reports the mean and maximum modeling errors for the tube and total models. We report the errors in percentage, as normalized with respect to the tube's (Tube Model) and total robot's (Total Model) length. We generally observe higher modeling errors related to the case of maximum bending of the tube. The highest is reported in Fig. \ref{fig:res_pics}(b), and its related to the case where the magnetic field is applied so that the chain can bend backward over the tube. This is the case of maximum physical instability and the position of the balls is not predicted as accurately as in Fig. \ref{fig:res_pics}(a). 

Overall, we observe that the proposed hybrid model, combination of Cosserat rod and magnetic energy minimization, is accurate enough (error $\leq$ 6\%) in predicting the robot's tip position.


\begin{table}[]
\centering
\caption{Results of model validation experiments.}
\label{table}
\begin{tabular}{l|c|c|}
\cline{2-3}
                                          & \textbf{Tube Model}                  & \textbf{Total Model}                 \\ \hline
\multicolumn{1}{|l|}{\textbf{Mean Error}} & 8.0mm (7.85\%)                        & 13.4mm (10.6\%)                      \\ \hline
\multicolumn{1}{|l|}{\textbf{Max Error}} & \multicolumn{1}{l|}{10.6mm (9.9\%)} & \multicolumn{1}{l|}{15.4mm (12.1\%)} \\ \hline
\end{tabular}
\end{table}


\subsection{Dexterous Workspace Demonstration}
To demonstrate how the hybrid design possesses a dexterous workspace as shown in Fig. 4, we placed a target in the dexterous portion of the workspace located along the main axis ($\pmb{z}$) of the catheter, and displaced 25mm upwards (axis $-\pmb x$). We then positioned the robot such that the tip touched the target from directions ranging over $2\pi$ in the two coordinate planes of Fig. 4(a) and 4(b). Four configurations are shown for the two planes in Fig. \ref{fig:target} illustrating that $\alpha_M = \beta_M = 2\pi$. Specifically in Fig. \ref{fig:target}(a) the catheter bends on the $\pmb x$-$\pmb z$ plane and different configurations of $\alpha_M$, are represented. Fig. \ref{fig:target}(b) shows different configurations of  $\beta_M$, with catheter bending happening on the $\pmb x$-$\pmb y$ plane. The maximum angle of about $2\pi$ is reached in Fig. \ref{fig:target}(a), subset \numcircled{4} and \ref{fig:target}(b), subset \numcircled{4}.
Figure \ref{fig:target} demonstrates that the hybrid continuum robots proposed here do have a dexterous workspace, even if the external magnetic field does not always suffice to fully straighten the ball chain. In particular, one can observe that the approximation becomes less accurate as the number of balls extended from the sheath increases. However, the range of reach angles respects the workspace analysis in Section \ref{sec:workspace}.
\begin{figure}[t]
    \centering
    \includegraphics{figures/target.png}
    \caption{Analysis of range approach angles (a) $\alpha_M$; and (b) $\beta_M$ for target within the dexterous workspace}. 
    \label{fig:target}
\end{figure}

==> sections/introduction.tex <==
Continuum robots have attracted considerable attention for applications in minimally invasive diagnostics and therapeutics over the past decade \cite{Dupont2022}. The primary reason is their ability to navigate narrow and tortuous anatomical passageways, while safely interacting with the anatomy. 

In designing such robots, an important goal is to create a robot with a workspace appropriate for the clinical task. A significant limitation of many continuum designs is that these robots lack a dexterous workspace. While clinical applications may necessitate approaching a target with a specific angle of approach, continuum designs are often limited in this regard. Furthermore, while multiple bending sections can be concatenated to provide more degrees of freedom, the orientations by which a point in the workspace can be approached are often highly constrained. 

To overcome this limitation, this paper investigates a hybrid design that combines the advantages of tendon-actuated  \cite{Rucker2011} and magnetic ball chain robots \cite{Pittiglio2023a} as shown in Fig. \ref{fig:hybrid}. In this hybrid design, a proximal tendon-actuated section positions the robot with respect to the goal tip location while a distal ball chain section orients the robot tip with respect to the goal location.% as shown in Fig. \ref{fig:main}.

This hybrid design is perhaps the only continuum robot possessing a true dexterous workspace - a continuous set of tip positions that can be approached from an arbitrary direction. The remainder of the paper is arranged as follows. The next two sections describe how kinematic models of varying complexity can be constructed for the tendon- and magnetically-actuated design. The subsequent section uses an approximate kinematic model to characterize the dexterous workspace. Section V contains an experimental validation of the kinematic model and workspace. Conclusions appear in the final section.

\begin{figure}[t]
    \centering
    \includegraphics[width = \columnwidth]{figures/main.png}
    \caption{Description of the hybrid tendon-actuated and magnetic ball-chain robot.}
    \label{fig:hybrid}
\end{figure}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width = 0.75\columnwidth]{figures/bladder.png}
%     \caption{Adding a retractable tendon-actuated tube to the ball chain steerable tip enables the robot to approach a tip position, $p$, from multiple tangent directions.}
%     \label{fig:main}
% \end{figure}

==> sections/inverse_kinematics.tex <==
In the prior section, a kinematic model was derived under the assumption that the ball chain does not deflect the proximal tendon-actuated tube. Even with this assumption, solution of the model involves solving a two-point boundary value problem and a constrained energy minimization problem. For purposes of design, workspace analysis and initialization of more complicated models, it is convenient to have a closed-form solution for the kinematics. 

We present such a model by making two additional simplifications. First, as explained in \cite{Rucker2011}, the constant-curvature model for a tendon-actuated tube in which the tendon load is approximated as a point moment at the tip is as accurate as the model of \cite{Rucker2011} for cases of no external load or loads applied in the plane of bending. This condition is satisfied based on our initial no-coupling assumption. 

Second, as noted in \cite{Pittiglio2023b}, the ball chain assumes a nearly linear shape aligned with the external magnetic field for sufficiently high field strengths. Under this assumption, it is possible to derive approximate closed-form forward and inverse kinematic models. Here, we present the inverse kinematic formulation. The forward equations can be easily derived from them. 

\subsection{Forward Kinematics}
The following notation is graphically explained in Fig. \ref{fig:hybrid}.
A ball chain robot is assumed to extend, for a length $l_c = n d_c$, as a straight line; here $n$ is the number of balls and $d_c$ their diameter. Given their base position and orientation in global reference frame, $^0\pmb p_b$ and $^0\pmb R_b$, their tip position and orientation is 
\begin{subequations}
\label{eq:chain_kin}
	\begin{align}
		\pmb p &={} ^0\pmb p_b + n d_c \ {}^0\pmb R_b \pmb{\omega}  \label{seq:chain_pos} \\
		\pmb R &= {}^0\pmb R_b \text{exp}\left(\pmb{\omega}_\times \right). \label{seq:chain_rot}
	\end{align}
\end{subequations}
The direction of the chain is a vector of norm 1, $\pmb{\omega} = \hat{\pmb B}$, and $\text{exp}(\pmb{\omega}_\times)$ the matrix exponential of $\pmb{\omega}_\times$.
We approximate the tendon-actuated continuum robot using constant curvature assumption, 
\begin{subequations}
\label{eq:tube_kin}
	\begin{align}
		\pmb p &={} ^0\pmb p_b + {}^0\pmb R_b \pmb{rot}_{\pmb e_3}(\phi)\pmb{w}   \label{seq:tend_pos} \\
		\pmb R &= {}^0\pmb R_b \pmb{rot}_{\pmb e_3}(\phi)\pmb{rot}_{\pmb e_2}\left(\frac{l_c}{\rho}\right) \label{seq:tend_rot}
	\end{align}
\end{subequations}
with $\pmb{w} = \rho \left(1 - \cos(l_c/\rho) \ 0 \  \sin(l_c/\rho) \right)^T$, $\rho$ and $l_c$ respective radius of curvature and length of the tendon-actuated continuum robot; $\pmb{rot}_{\pmb e_i}(\delta)$ is the rotation of the angle $\delta$ around the axis $\pmb e_i$.

By combining (\ref{eq:chain_kin}) with (\ref{eq:tube_kin}), we obtain the kinematics of the hybrid robot
\begin{subequations}
\label{eq:hyb_kin}
	\begin{align}
		\pmb p &={} ^0\pmb p_b + {}^0\pmb R_b \pmb{rot}_{\pmb e_3}(\phi)\pmb{w} + n d_c \pmb{rot}_{\pmb e_2}(\beta) \pmb \omega  \label{seq:hyb_pos} \\
		\pmb R &= {}^0\pmb R_b \text{exp}\left(\pmb{\omega}_\times \right) \label{seq:hyb_rot}
	\end{align}
\end{subequations}
Notice that, for any orientation of the tip of the tendon-actuated portion, the orientation of the chain's tip is dictated by the magnetic field direction.

\begin{figure*}[t]
    \centering
    \includegraphics[width = \textwidth]{figures/workspace.png}
    \caption{Description of the robot's dexterous workspace.}
    \label{fig:workspace}
\end{figure*}


\subsection{Inverse Kinematics}
The inverse kinematics problem is to solve for the set of inputs $\{F, \phi, \hat{\pmb B}\}$ for which the last ball of the chain approaches a goal position $\pmb p_g$ with orientation $\pmb v_g$ (see Fig. \ref{fig:inv_kin}). The input $F$ refers to the pulling force applied to the tendon, $\phi$ is the angular rotation around the main axis $\pmb z_b$, and $\hat{\pmb B}$ is the field orientation. 

First, we guarantee that the objective is feasible, i.e. we check if the point is reachable and the approach angles are within range. The distance from the axis is computed as $r = \sqrt{p_{g_x}^2 + p_{g_y}^2}$, and has to guarantee $r \leq r_d + nd_c$. The goal angle $\alpha_g$ and $\beta_g$ can be found as the twice the angle between $\pmb v_g$ and the respective axes $\pmb e_2$ and $\pmb e_3$: $\alpha_g = 2\arctan(\pmb v_g~\cdot \pmb e_2/||\pmb v_g\times \pmb e_2||)$ and $\beta_g = 2\arctan(\pmb v~\cdot \pmb e_3/||\pmb v_g\times \pmb e_3||)$. If $\alpha_g \leq \alpha_M(r)$ and $\beta_g \leq \beta_M(r)$, the inverse kinematics can be solved. The maximum range of orientations is defined in the next section.

In that case, the magnetic field orientation can be easily found as $\hat{\pmb B} = \pmb v_g$. Less intuitive is the solution for tendon-actuated robot. In this case, we search for the intersection between a line (the ball chain), extending from $\pmb p_g$ in the direction $- \pmb v_g$, and the cylinder of axis $\pmb e_3$ and radius $r_c$. This writes as
\begin{equation}
    \left\{
    \begin{array}{lcl}
    \pmb p(s) & = & \pmb p_g - \pmb v_g s  \\
    p_x^2(s) + p_y^2(s) & \leq & r_d \\
    ||\pmb v_g s|| \leq nd_c
    \end{array}
    \right.
\end{equation}
whose solution needs simultaneously satisfy
\begin{equation}
\label{eq:s_select}
\left\{
\begin{array}{ccccc}
      A - B & \leq & s & \leq & A + B \\
     && s & \leq & \frac{n d_c}{||\pmb v_g||}
\end{array}
\right.
\end{equation}
with
\begin{subequations}
\label{eq:constrains}
    \begin{align}
       A & = \frac{-p_{g_x} v_{g_x} + p_{g_y} v_{g_y}}{v_{g_x}^2 + v_{g_y}^2} \\
       B  & =  \frac{\sqrt{-(p_{g_x} v_{g_x} + p_{g_y} v_{g_y})^2 - r_d(v_{g_x}^2 + v_{g_y}^2)}}{v_{g_x}^2 + v_{g_y}^2}
       \end{align}
\end{subequations}

We can select any $s^*$ satisfying (\ref{eq:constrains}) and find the intersection point $\pmb p_i = \pmb p(s^*)$. 

We convert $\pmb p_i$ into cylindrical coordinates to find $\phi = \arctan(p_{i_y}/p_{i_x})$ and, from the direct kinematics in (\ref{eq:tube_kin}), we impose $\rho(1 - \cos(l_t/\rho)) = p_{i_x}$ and obtain $\rho = p_{i_x}/(1 - \cos(k))$, for some $k > 0$. Under constant curvature assumption \cite{Rao2021}, $\rho = \rho_i = \rho_j \ \forall i,j$ (see Fig. \ref{fig:inv_kin}), and the equilibrium is reduced to only bending moment $\pmb m = EI/\rho \pmb e_2$, constant along the robot's length. By applying the force $F$ along the tendon on the surface of the robot, we obtain the equilibrium $F d/2 \pmb e_2 = - EI/\rho \pmb e_2$ and find the pulling force
\begin{equation}
    F = -\frac{2EI(1 - \cos(k))}{dp_{i_x}}.
\end{equation}

The constant $k$ modulates between the length of the robot which can be inserted, depending on the anatomical site, and the amount of tension which can be applied to the tendon. These considerations are fundamental in the design for application-specific catheters.


==> sections/static_model.tex <==
A complete magneto-mechanical model considers the interaction between the tendon-driven tube and the magnetically actuated ball chain, relaxing the assumptions of Section \ref{sec:workspace}. Specifically, the assumption that the tube bends as a 
constant curvature element and that the ball chain follows a straight line. By combining the results in \cite{Rucker2011} and \cite{Pittiglio2023a}, we discuss a solution to the static equilibrium.

In the following, we assume that there is no friction between the ball chain and the tube.% and that the latter is rigid enough to constrain the balls' tendency to align. We also consider that the tube's elastic behaviour is linear and that the tendon is constrained to run parallel to the tube. 

\subsection{Mechanical Model}
\label{sub:mech_mod}
% \begin{figure}
%     \centering
%     \includegraphics{figures/mech_model.png}
%     \caption{Description of the load on the tendon actuated tube.}
%     \label{fig:mech_model}
% \end{figure}
The centerline of the tube can be described, in function of its length parameter $s \in \left[0, l_t\right]$ with its position $\pmb p_c(s) \in \mathbb{R}^3$ and orientation $\pmb R_c(s) \in SO(3)$,
\begin{subequations}
\label{eq:tube_cent}
    \begin{align}
    \dot{\pmb p}_c(s) &= \pmb R_c(s) \pmb v(s) \\
    \dot{\pmb R}_c(s) &= \pmb R_c(s) \pmb u_\times(s)
   \end{align}
\end{subequations}
where $\pmb v(s) \in \mathbb{R}^3$ and $\pmb u(s) \in \mathbb{R}^3$ are the respective linear and angular strain. Following the Cosserat rod modeling \cite{Rucker2011}, we describe the internal forces $\pmb n$ and moments $\pmb m$ with respect to the applied force $\pmb f$ and torque $\pmb \tau$ as
\begin{equation}
\label{eq:int_forces}
\left(
\begin{array}{c}
    \dot{\pmb n}  \\
     \dot{\pmb m} 
\end{array}
\right)
= 
\left(
\begin{array}{cc}
    \pmb u_\times & \pmb 0 \\
    \pmb v_\times & \pmb{u}_\times
\end{array}
\right)
\left(
\begin{array}{c}
    \pmb n  \\
    \pmb m
\end{array}
\right)
+ 
\left(
\begin{array}{c}
    \pmb f  \\
    \pmb \tau
\end{array}
\right)
\end{equation}
Under assumption of linear elasticity, we have
\begin{equation}
    \left(
\begin{array}{c}
    \pmb n  \\
    \pmb m
\end{array}
\right) = K 
\left(
\begin{array}{c}
    \pmb u - \pmb{u}_0 \\
    \pmb v - \pmb{v}_0
\end{array}
\right)
\end{equation}
with $K = diag(GA, GA, EA, EI_{xx}, EI_{yy}, GJ_{zz})$, where $G$ is the shear modulus, $E$ modulus of elasticity, $A$ cross-sectional area, $I_{xx}$, $I_{yy}$  second moment of area around the $\pmb x$ and $\pmb y$ axes, and $J_{zz}$ the polar moment of area; $\pmb{u}_0$ and $\pmb{v}_0$ are the initial linear and angular strain respectively.

The tube is subject to three main external inputs: distributed force related to the force applied by the tendon at the tip  $\pmb f_t$; gravitational force $\pmb f_g = m \pmb g$, $m$ mass density and $\pmb g$ gravitational acceleration; and external forces applied by the magnetic ball chain.

Following \cite{Rucker2011}, the path of the tendon on the surface of the tube along the $\pmb x$ axis is
\begin{equation}
    \pmb p_t(s) = \pmb p_c(s) + \frac{d_t}{2} \pmb R_c(s) \pmb{e}_1
\end{equation}
and the relative force is
\begin{equation}
    \pmb f_t = -\lambda \frac{\dot{\pmb{p}}^2_{t_\times}}{\|\pmb{p}_{t}\|^3}\ddot{\pmb p}_t
\end{equation}
with $\lambda$ tension applied to the tendon.

The load applied by the ball chain can be subdivided into a point load at the tip, due to gravity and forces applied to the extending section of the chain, point force applied to the tube at the point of contact with the balls. We consider that, at any instant, $n_e$ balls, of the $n$ total number of balls, extend from the tendon-actuated tube. The force applied to the extending balls is the resultant of the applied magnetic field and gravity
\begin{equation}
    \pmb f_e = \sum_{i = 1}^{n_e} \sum_{k = 1}^2 \pmb R^T_c(l_t) \pmb e_k^T\left(\pmb f_{b_j} + m_j\pmb g\right) \pmb R_c(l_t) \pmb  e_k
\end{equation}
with $\pmb f_{b_j} = \nabla(\pmb \mu_j \cdot \pmb B(\pmb p_j))$ magnetic force, where $\pmb \mu_j \in \mathbb{R}^3$ is the magnetic dipole vector of the $i$th ball $\pmb{p}_j$ its position and $m_j$ its mass. Since we assume no friction between the ball chain and the tube, the chain exerts forces on the tube only on the cross-sectional plane. 

The forces generated by the section of the chain internal to the tube can be considered as point forces related to the force applied to each ball and the force generated by each ball rotating with respect to the previous one. In fact, as we apply a magnetic torque on the $i$th ball $\pmb \tau_{b_i}$, its tendency to rotate  with respect of the previous ball generates a force on the tube equal to $\pmb \tau_{b_i} \times \pmb R_c(s_i)\pmb e_3/d$, at the point of coordinate $s = s_i = l_t - (n - n_e - i)d$. When we sum it to magnetic forces applied by the other balls $k \neq i$ and from the external field, we obtain the point force applied by the $i$th ball onto the tendon-actuated catheter 
\begin{eqnarray}
\label{eq:mag_force}
        \pmb f_{b_i}(s_i) &=& \sum_{k \neq i} \sum_{h = 1}^2 \pmb R^T_c(s_i) \pmb e_h^T\bigl(\nabla(\pmb \mu_j \cdot \pmb B(\pmb p_i)\nonumber \\
        && + \nabla(\pmb \mu_j \cdot \pmb B_k(\pmb p_i)) \bigl) \pmb R_c(s_i)\pmb e_h \nonumber \\  
        && + \pmb \mu_i \times(\pmb B(\pmb p_i) + \pmb B_k(\pmb p_i))) \nonumber \\
        && \times \pmb R_c(s_i) \pmb e_3/d 
\end{eqnarray}
with $p_i = p(s_i)$.
At each balls location, we sum the force with the gravitational force and obtain the overall force $\pmb f_i(s_i) = \pmb f_{b_i}(s_i) + m_i\pmb g$.

\subsection{Magnetic Model}
\label{sub:mag_mod}
The magnetic equilibrium can be solved by following \cite{Pittiglio2023a, Pittiglio2023b}, as a constrained energy minimization problem, where the energy is combination of magnetic, elastic, and gravitational components as
\begin{subequations}
\label{eq:energies}
    \begin{align}
        U_b &= -\sum_{i = 1}^n \sum_{j = i + 1}^n {} \pmb{\mu}_j \cdot \pmb{B}_j(\pmb{p}_i) \\
        U_s &=  \frac{1}{2}\sum_{i = 1}^{n - n_e} \frac{E_t I_t \theta_i}{\rho_i} + \frac{1}{2}\sum_{n - n_e + 1}^n \frac{E_s I_s \theta_i}{\rho_i} \\
        U_g &= \sum_{i = 1}^n m_i \pmb{g}^T \pmb{p}_i,
    \end{align}
\end{subequations}
where $E_t$ and $E_s$ are the elastic modulus of the tube and sleeve, respectively. In (\ref{eq:energies}), as in \cite{Pittiglio2023a, Pittiglio2023b}, we have considered the discrete nature of the chain and discretized the radius of curvature $\rho_i$ and bending angle $\theta_i$ (see Fig. \ref{fig:inv_kin}) between consecutive balls. As discussed in the following, when combining this approach with the Cosserat rod model in Section \ref{sub:mech_mod}, we obtain a full solution which does not assume constant curvature between spheres.

By combining the terms in (\ref{eq:energies}), we obtain the total energy $U = U_b  + U_s + U_g$.

\subsection{Solution of the Combined Model}
We combine the models in Section \ref{sub:mech_mod} and \ref{sub:mag_mod} by solving the differential equations iteratively. First, we consider the tendon-actuated tube can bend without the presence of magnetic balls and solve the Cosserat model equations with distributed load applied to  (\ref{eq:int_forces})
\begin{subequations}
\label{eq:mech_load}
    \begin{align}
        \pmb f &= \pmb f_t + m\pmb g \\
        \pmb \tau &= (\pmb p(s) - \pmb p_t(s)) \times \pmb f_t
    \end{align}
\end{subequations}
and force and torque boundary conditions at the tip
\begin{subequations}
\label{eq:mech_bound}
\begin{align}
    \pmb F(l_t) &= -\lambda \frac{\dot{\pmb p}_c(l_t)}{\|\dot{\pmb p}_c(l_t)\|} \\
    \pmb T(l_t) &= (\pmb p_c(l_t) - \pmb p_t(l_t)) \times \pmb F(l_t).
\end{align}
\end{subequations}
We obtain the position and orientation of the centerline $\pmb p^*_c(s)$ and $\pmb R^*_c(s)$, solution of the differential equations, and $(\pmb{u}_0^*$, $\pmb{v}_0^*)$, the linear and angular strain. The centerline is discretized to obtain the initial position and dipole of each sphere inside the tube 
\begin{subequations}
\label{eq:init_cond1}
    \begin{align}
        \pmb p_{0_i} &= \pmb p_c(l_t - (n - n_e - i)d), \ i = 1, 2, \dots, n - n_e \\
        \pmb \mu_{0_i} &= \|\mu\| \pmb R_c(l_t - (n - n_e - i)d) \pmb e_3,  \ i = 1, 2, \dots, n - n_e
    \end{align}
\end{subequations}
with $\|\mu\|$ magnetic dipole strength of the balls. The position and dipole of the remaining balls $n-n_e < j \leq n$ was found applying (\ref{eq:chain_kin}), i.e. we assume they follow a straight line in the field direction. 
\begin{subequations}
\label{eq:init_cond2}
    \begin{align}
        \pmb p_{0_j} &= \pmb p_c(l_t) + j d \pmb R_c(l_t) \pmb e_3, \ j = n - n_e + 1, \dots, n \\
        \pmb \mu_{0_j} &= \|\mu\| \pmb R_c(l_t) \pmb e_3, \ j = n - n_e + 1, \dots, n
    \end{align}
\end{subequations}
Using $( p_{0_j}, \mu_{0_j})$ as initial guess, we solve the minimization problem
\begin{equation}
\label{eq:optimization}
(\pmb{p}_i^*, \pmb \mu_i^*), \ i \in 2, \ldots, n = \argmin_{(\pmb{p}_i, \pmb \mu_i), \ i \in 2, \ldots, n} U
\end{equation}
using the Matlab (Mathworks, Natick, MA) routine {\it fmincon}. The imposed constraints result from assuming continuous contact between subsequent balls over time and constant dipole intensity, i.e.
\begin{subequations}
\label{eq:constraints}
    \begin{align}
        \|\pmb{p}_i\| &= d \ \forall \ i=1,2,\dots,n.\\
        \|\pmb{\mu}_i\| &= \|\pmb{\mu}\| \ \forall \ i=1,2,\dots,n. \\
        \pmb{\mu}_1 &= \pmb e_3
    \end{align}
\end{subequations}
The last constraint is to force the first ball to be aligned with the chain's axis. In the real setup, this is achieved by gluing.

The last step is to apply the magnetic load, resulting from the solution of the energy minimization, to the tube. From the deflection $(\pmb u_0^*, \pmb v_0^*)$, with no distributed load, we apply the boundary conditions \cite{Rao2021}
\begin{equation}
\label{eq:mag_bound}
    \pmb{n}(s_i^-) = \pmb{n}(s_i^+) + \pmb f_{b_i}(s_i) + m_i \pmb{g},
\end{equation}
$\pmb f_{b_i}(s_i)$ is derived in (\ref{eq:mag_force}).

This process is run iteratively, until $(\dot{\pmb{n}}, \dot{\pmb{m}}) \leq \epsilon \approx 0$, as described in Algorithm \ref{alg:optimization}.

\begin{algorithm}
\caption{Solution of the static equilibrium.}
\label{alg:optimization}
\While{$(\dot{\pmb{n}}, \dot{\pmb{m}}) > \epsilon$}{
    $(\pmb{u}_0, \pmb v_0) \gets (0, 0)$\;
    $(\pmb f, \pmb \tau)$ \text{defined in} (\ref{eq:mech_load})\;
    Boundary conditions in (\ref{eq:mech_bound})\;
    $(\pmb p_c', \pmb R_c', \pmb{u}^*_0, \pmb v^*_0) \gets$ Solve (\ref{eq:int_forces})\;
    $(\pmb{p}_{i_0}, \pmb \mu_{i_0}) \gets$ Eqs. (\ref{eq:init_cond1})-(\ref{eq:init_cond2})\;
    Constraints in (\ref{eq:constraints})\;
    $(\pmb{p}_i^*, \pmb \mu_i^*)\gets$ Solve (\ref{eq:optimization})\;
    $(\pmb f, \pmb \tau) \gets$ (0, 0)\;
    Boundary conditions in (\ref{eq:mag_bound})\;
    $(\pmb p_c^*, \pmb R_c^*, \dot{\pmb{n}}, \dot{\pmb{m}}) \gets$ Solve (\ref{eq:int_forces})\;
}
\end{algorithm}

\subsection{Practical Considerations and Simplifications}
In our case, which we will show with some experiments in the following section, the tendon actuated section is stiff enough for the effect of the internal balls to be negligible to the equilibrium of the tube. The consequence is that we see that Algorithm \ref{alg:optimization} converges after one iteration to an accurate solution. This implies that we can simplify the algorithm by: avoiding iteration and accepting $(\pmb p_c^*, \pmb R_c^*) = (\pmb p_c', \pmb R_c')$ as solution to the centerline of the tube; simplify $U_s =  \frac{1}{2}\sum_{n - n_e + 1}^n \frac{E_s I_s \theta_i}{\rho_i}$ and convert the elastic energy of the tube into the set of constraints
\begin{subequations}
\label{eq:constraints_simp}
    \begin{align}
        \pmb{p}_i &= \pmb{p}_{i_0} \ \forall \ i=1,2,\dots,n - n_e.\\
        \pmb{\mu}_i &= \pmb{\mu}_{i_0} \ \forall \ i=1,2,\dots,n - n_e.
    \end{align}
\end{subequations}
These simplifications do not notably change the results of the algorithm, but reduce its complexity and computational time significantly. Experimentally, we computed the difference between the position of the tip of the tube with ball chain inside, without ball chain and with extended ball chain with applied field, as presented in Section \ref{sec:experiments}. In the next section, we characterize the error related to this assumption.

==> sections_v2/static_model.tex <==
A complete mechanics-based model of the hybrid design can be derived by combining the tendon-actuated model of  \cite{Rucker2011} with the magnetic energy ball-chain model of \cite{Pittiglio2023a}. In this approach, the magnetic balls retracted inside the tendon-actuated tube exert ``external'' point loads on the tube while the extended portion of the ball chain exerts a tip force on the tube. The magnitudes of these forces can be computed using the formulation of \cite{Pittiglio2023a}, but depend on the deflected tube shape. An iterative  approach can be used to alternately solve the tube and ball chain models until convergence is reached. 

If the forces from the magnetic ball chain do not appreciably deflect the tendon-actuated tube, the kinematic modeling equations and solution procedure can be substantially simplified and solved in a single iteration. In this case, the tendon-actuated tube shape can be computed first. The position constraints from the tube shape can then be imposed on the ball chain to solve for the shape of its extended portion. When this simplification can be applied, it is advantageous since the model becomes less complex and the computation time faster. Since initial experiments with our prototype system described later in the paper match this behavior, the simplified model is considered here. 

The following subsections summarize the tendon-actuated tube model and the magnetic energy ball chain model.

\subsection{Tendon-actuated tube}
\label{sub:mech_mod}
% \begin{figure}
%     \centering
%     \includegraphics{figures/mech_model.png}
%     \caption{Description of the load on the tendon actuated tube.}
%     \label{fig:mech_model}
% \end{figure}
The centerline of the tube can be described, as a  function of arc-length, $s \in \left[0, l_t\right]$, with its position $\pmb p_c(s) \in \mathbb{R}^3$ and orientation $\pmb R_c(s) \in SO(3)$,
\begin{subequations}
\label{eq:tube_cent}
    \begin{align}
    \dot{\pmb p}_c(s) &= \pmb R_c(s) \pmb v(s) \\
    \dot{\pmb R}_c(s) &= \pmb R_c(s) \pmb u_\times(s)
   \end{align}
\end{subequations}
where $\pmb v(s) \in \mathbb{R}^3$ and $\pmb u(s) \in \mathbb{R}^3$ are the respective linear and angular strain; the ``skew" operator is defined as $\pmb{u}_\times = \left(\pmb{u} \times \pmb e_1  \ \pmb{u} \times \pmb e_2 \ \pmb{u} \times \pmb e_3  \right)$ with $\pmb e_i\in \mathbb{R}^{3}$ $i$th element of the canonical basis of $\mathbb{R}^3$, $\times$ indicating the cross product. Here, the dot notation is used to indicate derivatives with respect to arc-length (i.e. $\dot{\pmb p}_c(s) = \frac{d{\pmb p}_c(s)}{ds}$). Following the Cosserat rod modeling \cite{Rucker2011}, we describe the internal forces $\pmb n$ and moments $\pmb m$ with respect to the applied force $\pmb f$ and torque $\pmb \tau$ as
\begin{equation}
\label{eq:int_forces}
\left(
\begin{array}{c}
    \dot{\pmb n}  \\
     \dot{\pmb m} 
\end{array}
\right)
= 
\left(
\begin{array}{cc}
    \pmb u_\times & \pmb 0 \\
    \pmb v_\times & \pmb{u}_\times
\end{array}
\right)
\left(
\begin{array}{c}
    \pmb n  \\
    \pmb m
\end{array}
\right)
+ 
\left(
\begin{array}{c}
    \pmb f  \\
    \pmb \tau
\end{array}
\right)
\end{equation}
Under assumption of linear elasticity, we have
\begin{equation}
    \left(
\begin{array}{c}
    \pmb n  \\
    \pmb m
\end{array}
\right) = K 
\left(
\begin{array}{c}
    \pmb u - \pmb{u}_0 \\
    \pmb v - \pmb{v}_0
\end{array}
\right)
\end{equation}
with $K = diag(GA, GA, EA, EI_{xx}, EI_{yy}, GJ_{zz})$, where $G$ is the shear modulus, $E$ modulus of elasticity, $A$ cross-sectional area, $I_{xx}$, $I_{yy}$  second moment of area around the $\pmb x$ and $\pmb y$ axes, and $J_{zz}$ the polar moment of area; $\pmb{u}_0$ and $\pmb{v}_0$ are the initial angular and linear strain respectively.

The tube is subject to two main external inputs: distributed force related to the force applied by the tendon at the tip  $\pmb f_t$; and gravitational force $\pmb f_g = m \pmb g$, $m$ mass density and $\pmb g$ gravitational acceleration.

Following \cite{Rucker2011}, the path of the tendon on the surface of the tube along the $\pmb x$ axis is
\begin{equation}
    \pmb p_t(s) = \pmb p_c(s) + \frac{d_t}{2} \pmb R_c(s) \pmb{e}_1
\end{equation}
and the relative force and torque are
\begin{subequations}
\begin{align}
     \pmb f_t &= -\lambda \frac{\dot{\pmb{p}}^2_{t_\times}}{\|\pmb{p}_{t}\|^3}\ddot{\pmb p}_t \\
     \pmb{\tau}_t &= \pmb{p}_t \times \pmb f_t
\end{align}
\end{subequations}
with $\lambda$ tension applied to the tendon and $d_t$ is the diameter of the tube.

The load at the tip is implemented as a boundary condition,
\begin{subequations}
\label{eq:mech_bound}
\begin{align}
    \pmb F(l_t) &= -\lambda \frac{\dot{\pmb p}_c(l_t)}{\|\dot{\pmb p}_c(l_t)\|} \\
    \pmb T(l_t) &= (\pmb p_c(l_t) - \pmb p_t(l_t)) \times \pmb F(l_t).
\end{align}
\end{subequations}

\subsection{Magnetic ball chain}
\label{sub:mag_mod}
The equilibrium configuration of the magnetic ball chain can be solved by minimizing the potential energy of the system. Following \cite{Pittiglio2023a, Pittiglio2023b}, the total potential energy of the balls can be expressed as a combination of magnetic and gravitational components as 
\begin{subequations}
\label{eq:energies}
    \begin{align}
       U_{e} &= -\sum_{i = 1}^n {} \pmb{\mu}_i \cdot {} \pmb{B}(\pmb{p}_i - \pmb{p}_e, \pmb{\mu}_e ) \label{seq:ext_mag} \\
        U_b &= -\sum_{i = 1}^n \sum_{j = i + 1}^n {} \pmb{\mu}_i \cdot \pmb{B}(\pmb{p}_i -\pmb{p}_j, \pmb{\mu}_j ) \label{seq:int_mag} \\ 
        U_g &= \sum_{i = 1}^n m_i \pmb{g}^T \pmb{p}_i, \label{seq:grav}
    \end{align}
\end{subequations}
In (\ref{seq:ext_mag}), we express the interaction with the external magnet in position $\pmb p_e$ and magnetic dipole $\pmb \mu_e$, (\ref{seq:int_mag}) considers the intermagnet energy for the magnets in the chain, and (\ref{seq:grav}) is the gravitational component. The magnetic field is computed using the dipole model
$$\pmb{B}(\pmb{r}, \pmb{\mu}) = \frac{ \mu_0}{4 \pi |\pmb{r}|^3} \left(3 \hat{\pmb{r}} \hat{\pmb{r}}^T - I \right) \pmb{\mu}.$$

By combining the terms in (\ref{eq:energies}), we obtain the total energy $U = U_e + U_b  + U_g$.
In \cite{Pittiglio2023a},  we have considered the discrete nature of the chain and discretized the radius of curvature $\rho_i$ and bending angle $\theta_i$ (see Fig. \ref{fig:inv_kin}) between consecutive balls, to consider elastic terms in the sleeve containing the chain. In contrast to our prior work, we solve for the minimum energy configuration while constraining the position of the $n_i$ balls inside the tube using Matlab function {\it fmincon}, since the tube can be considered infinitely stiff, in this case. These constraints are given by 
\begin{equation}
\label{eq:constraints_simp}
        \pmb{p}_i = \pmb{p}_{i_0} \ \forall \ i=1,2,\dots,n_i
\end{equation}
$\pmb{p}_{i_0}$ is derived from the the Cosserat equilibrium.

As in our previous work \cite{Pittiglio2023b}, we constrain each ball to be in continuous contact with the previous one and the dipole intensity of the $n$ balls to be constant
\begin{subequations}
    \begin{align}
        \|\pmb{p}_i - \pmb{p}_{i-1}\| &= d \ \forall \ i=2,3,\dots,n. \\
        \|\pmb{\mu}_i\| &= \mu \ \forall \ i=1,2,\dots,n.
    \end{align}
\end{subequations}
The overall solution is obtained by first solving for the shape of the tendon-actuated tube and then using its position to solve for the shape of the ball chain. 

\begin{figure}[t]
    \centering
    \includegraphics[width = \columnwidth]{figures/inv_kin.png}
    \caption{Description of the model for hybrid tendon actuated and ball chain robots.}
    \label{fig:inv_kin}
\end{figure}



